Distributed-Memory Parallel Algorithms for Fixed-Radius Near Neighbor Graph Construction

Computing fixed-radius near-neighbor graphs is an important first step for many data analysis algorithms. Near-neighbor graphs connect points that are close under some metric, endowing point clouds with a combinatorial structure. As computing power and data acquisition methods advance, diverse sources of large scientific datasets would greatly benefit from scalable solutions to this common subroutine for downstream analysis. Prior work on parallel nearest neighbors has made great progress in problems like k-nearest and approximate nearest neighbor search problems, with particular attention on Euclidean spaces. Yet many applications need exact solutions and non-Euclidean metrics. This paper presents a scalable sparsity-aware distributed memory algorithm using cover trees to compute near-neighbor graphs in general metric spaces. We provide a shared-memory algorithm for cover tree construction and demonstrate its competitiveness with state-of-the-art fixed-radius search data structures. We then introduce two distributed-memory algorithms for the near-neighbor graph problem, a simple point-partitioning strategy and a spatial-partitioning strategy, which leverage the cover tree algorithm on each node. Our algorithms exhibit parallel scaling across a variety of real and synthetic datasets for both traditional and non-traditional metrics. On real world high dimensional datasets with one million points, we achieve speedups up to 678.34x over the state-of-the-art using 1024 cores for graphs with 70 neighbors per vertex (on average), and up to 1590.99x using 4096 cores for graphs with 500 neighbors per vertex (on average).

==> section/discussion.tex <==
\section{Discussion}

\todo[inline]{Discuss problems encountered with load imbalance}
Load balancing is a major challenge with geometric algorithms. Using the number of points in a Voronoi cell as a runtime estimate does not work for two separate reasons: first, the expansion constant of different subsets of points can vary widely, which leads to poor 
\todo[inline]{Discuss problems with load balancing algorithm related to inefficient communication strategy and problem with large counts and how to overcome}
\todo[inline]{Discuss problems with Voronoi cell site selection in terms of load imbalance and how to overcome}
\todo[inline]{Discuss problems with Voronoi cell site computation in terms of compute-bound distance computations, potential for acceleration using GPUs and also a recursive decomposition into subcommunicators}
\todo[inline]{Discuss inefficiencies in ghost point communication}
\todo[inline]{Discuss shortcomings with datasets and lack of non-Euclidean results for a paper claiming non-Euclidean as an important motivator..}

==> section/junk.tex <==
\section{Algorithm}
Let $P$ be a set of $n$ points from a metric space $X$ with distance function $d$. Let $m < n$ be the number of sites in our ``greedy net''. Specifically, we seek $m$ points $p_1, \ldots, p_m \in P$ such that $d(p_i,p_j) \geq \gamma$ for all $i \neq j$ and some $\gamma > 0$, and such that $d(p, p_i) \leq \gamma$ for all $p \in P$ such that $p_i$ is the closest of the $m$ sites to $p$. Let $V(p_i)$ denote the Voronoi cell associated with the site $p_i$:
$$V(p_i) = \{p \in P : d(p,p_i) = d(p, P_m)\}.$$

%\section{Brainstorm}
%Let $P$ be a set of $n$ metric points. Let $P_m = \{p_1, \ldots, p_m\} \subset P$ be a subset of $m$ points from $P$, where $m \ll n$.
%Let $$V_i = \{p \in P : d(p,p_i) = d(p,P_m)\}$$ be the Voronoi cell associated with $p_i \in P_m$, i.e. the set of points in $P$ that are closer to $p_i$ than they are to any of the other points in $P_m$.
%The initial idea is to distribute Voronoi cells to processors and to build local cover trees $T_i$ on the set of points in $V_i$, for each $p_i \in P_m.$ We then would find all $\epsilon$-neighbors of a point $p \in P$ by finding its Voronoi cell $V_i$, and querying $T_i$ for its neighbors. To do this in parallel, we would have each processor go through its assigned set of Voronoi cells $V_i$ and query all the points in $V_i$ against $T_i$ to compute $B(p, \epsilon).$
%We run into a common problem in parallel algorithms with this approach. Not all $\epsilon$-neighbors of a point $p \in V_i$ are going to be in $V_i$. We therefore need to add ``ghost points'' to $V_i$ that originate in other Voronoi cells.
%
%
%Suppose we are trying to find $\epsilon$-neighbors of $p \in V_i$. Let $q \in V_j$ be an $\epsilon$-neighbor of $p$ in a different Voronoi cell, i.e. $i \neq j$.
%Then $d(q,p_i) \leq d(p,q) + d(p,p_i)$ by triangle inequality. We know $d(p,p_i) \leq d(p,p_j)$ since $p \in V_i$, therefore we get $d(q,p_i) \leq d(p,q) + d(p,p_j).$ Again applying triangle inequality, we get $d(q,p_i) \leq 2d(p,q) + d(q,p_j)$. Therefore we know for a fact that
%$$d(q,p_i) \leq d(q,p_j) + 2\epsilon.$$
%
%Let's use this to adjust our initially incorrect approach. Let $G_i^\epsilon$ denote the set of potential $\epsilon$-neighbors of points in $V_i$ which do not belong to $V_i$ themselves. That is:
%$$G_i^\epsilon = \{p \in P \setminus V_i : d(p,p_i) \leq d(p,P_m) + 2\epsilon\}.$$
%We then build local cover trees $T_i$ in the set of points $V_i \cup G_i^\epsilon$. Then, we simply go through each local $T_i$, and query all points in $V_i$ against $T_i$. This is guaranteed to find all $\epsilon$-neighbors.
%
%\section{Introduction}
%
%
%There is a significant literature dedicated toward the development of fast nearest neighbor search algorithms. The classic algorithms, first developed in the 70s, used a tree data structure to decompose the points into subsets satisfying desirable geometric invariants which answer queries in a recursive fashion. Finkel and Bentley introduced the Quadtree in 1974~\cite{finkel74}, and Bentley shortly thereafter developed the kd-tree~\cite{bentley75}.
%These data structures have proven to be highly efficient solutions to proximity search and $k$-nearest neighbors search in low-dimensional Euclidean metric spaces. However, these data structures require the underlying metric to be Euclidean, and are notoriously inefficient in higher dimensional spaces. Alternative structures such as the ball tree~\cite{omohundro89} attempted to deal with the curse of dimensionality, but were still only applicable to Euclidean points.
%Uhlmann (and Yianilos, independently) developed vantage-point trees (vp-trees) in the early 90s that worked on general metric spaces~\cite{uhlmann91, yianilos93}.
%All these data structures cut the average number of distance computations from $O(n^2)$ down to $O(n\log{n})$ (CONFIRM THIS).
%
%To be continued...
%
%
%The purpose of this work is to develop a high performance distributed-memory algorithm that 
%computes $\epsilon$-graphs. $\epsilon$-graphs are commonly used structures in computational geometry. Many important algorithms in Topological Data Analysis (TDA) make use of $\epsilon$-graphs, which is one of the major motivating factors behind our research. At the most general level, we are given a set of $n$ points $P$ from some metric space $(X,d).$ An $\epsilon$-graph on $P$ is an undirected graph $G = (V,E)$ where $V = P$ and $E = \{(p,q) : d(p,q) \leq \epsilon\}.$
%In words, each vertex in the graph is a point in $P$, and we insert an edge between every pair of vertices that are within a distance of $\epsilon$ of each other.
%The obvious naive solution can be computed using $O(n^2)$ distance computations, by going through all $n \choose 2$ pairs, computing their distance, and recording the edges that are within $\epsilon$ distance of each other. With $N$ processors, this is trivially $O(n^2/N)$, assuming all processors have access to all the points.
%
%
%\section{Overview}
%We now give a high-level overview of a parallel strategy to construct $\epsilon$-graphs. To avoid confusion, we assume that $M$ is the set of $n$ points we want to build a graph for, and that $P$ is the number of processors.


\section{Algorithm}

\begin{definition}
    A \textbf{metric space} $(X,d)$ is a set of points $X$ along with a distance function $d : X \times X \to \mathbb{R}$ such that for all $x,y,z \in X$
    \begin{itemize}
        \item[(i)] $d(x,y) \geq 0$ (distances are nonnegative),
        \item[(ii)] $d(x,y) = 0$ if and only if $x = y$ (distance to self is $0$),
        \item[(iii)] $d(x,y) = d(y,x)$ (distances are symmetric), and
        \item[(iv)] $d(x,y) \leq d(x,z) + d(z,y)$ (triangle inequality).
    \end{itemize}
    Any finite subset of $X$ is a \textbf{finite metric space}. We assume all of our metric spaces are finite from now on.
\end{definition}

%\noindent For any subset $S \subset X$, the distance between a point $p$ and the set $S$ is the distance between $p$ and its nearest neighbor in $S$. That is, $d(p,S) = \min_{x \in S}d(p,x).$
%
%\begin{definition}
%    Let $(X,d)$ be a metric space. The \textbf{(closed) ball} in $X$ with center $p \in X$ and radius $r \geq 0$ is the set $$B(p,r) = \{x \in X : d(p, x) \leq r\}.$$
%    We denote the set of balls of radius $r$ centered at the points of $P \subset X$ by $$\mathcal{B}(P, r) = \bigcup_{p \in P}B(p, r).$$
%\end{definition}
%
%\begin{definition}
%    Let $P$ be a set of points and $S \subset P$ be a subset of $P$. The \textbf{coverage radius} of $S$ with respect to $P$, denoted $\mathcal{C}_P(S)$, is the minimum value $r \geq 0$ such that $P \subset \mathcal{B}(S,r)$. It is easy to see that $\mathcal{C}_P(S) = \max_{p \in P}d(p,S)$.
%\end{definition}
%
%\begin{definition}
%    Let $P$ and $S$ be subsets of a metric space $(X,d)$. The \textbf{Hausdorff distance} between $P$ and $S$ is the largest distance possible between a point in $P$ or $S$ and the nearest neighbor in the other set. That is,
%    $$d_H(S,P) = \max\{\max_{p \in P}d(p,S), \max_{x \in S}d(x,P)\}.$$
%    This is the same as the minimum value $r \geq 0$ such that $P \subset \mathcal{B}(S,r)$ and $S \subset \mathcal{B}(P,r).$ If $S$ is a subset of $P$, then $d_H(S,P) = \mathcal{C}_P(S).$
%\end{definition}
%
%\begin{definition}
%    Again let $P$ be a set of points. The \textbf{minimum separation} of $P$, denoted by $\mathcal{S}(P)$, is the minimum pairwise distance between points in $P$. That is,
%    $$\mathcal{S}(P) = \min_{p \neq q \in P}d(p,q).$$
%\end{definition}
%
%\begin{definition}
%    The \textbf{diameter} of a set of points $P$, denoted by $\mathcal{D}(P)$, is the maximum pairwise distance between points of $P$. That is, $$\mathcal{D}(P) = \max_{p, q \in P}d(p,q).$$
%\end{definition}
%
%\begin{definition}
%    The \textbf{spread} of a set of points $P$, denoted by $\Delta(P)$, is the ratio of the diameter and minimum separation of $P$. That is, $$\Delta(P) = \frac{\mathcal{D}(P)}{\mathcal{S}(P)}.$$
%    The spread is alternatively called the \textbf{aspect ratio} in the literature.
%\end{definition}
%
%\begin{definition}
%Let $(X,d)$ be a metric space. We say that $X$ has \textbf{doubling dimension} $\rho = \mathrm{dim}(X)$ if $\rho$ is the smallest constant value such that for all $x \in X$ and all $r > 0$, there exists $y_1, y_2, \ldots, y_m \in X$ such that $m \leq 2^{\rho}$ and
%$$B(x,2r) \subset \bigcup_{i=1}^{m}B(y_i, r).$$
%\end{definition}
%
%\begin{definition}
%Let $(X,d)$ be a finite metric space. We say that $X$ has \textbf{expansion constant} $c$, with $\log_{2}{c} = \mathrm{dim}_{KR}(X)$, if $c$ is the smallest constant such that for all $x \in X$ and $r > 0$, we have
%$$|B(x,2r)| \leq c\cdot|B(x,r)|.$$l
%\end{definition}
%
%\begin{definition}
%    Let $S \subset P$. $S$ is called an \textbf{$r$-net} for $P$ if it has coverage radius at most $r$ and minimum separation at least $r$.
%\end{definition}
%
%\begin{definition}
%    Let $P$ be a set of $n$ points with an ordering $(p_1, p_2, \ldots, p_n).$ Let $P_i = \{p_1, \ldots, p_i\}$ be the prefix with $i$ points. The ordering is a \textbf{greedy permutation} if for each $1 \leq i < n$, the next point $p_{i+1}$ in the sequence is the farthest point from $P_i.$ That is, $d(p_{i+1}, P_i) \geq d(p, P_i)$ for all $p \in P$. The first point $p_1$ is arbitrarily chosen.
%\end{definition}
%
%
%\begin{lemma}
%    Let $P = (p_1, \ldots, p_n)$ be a greedy permutation and let $r_k = d(p_{k+1}, P_k)$ for $k < n$ and $r_n = 0.$ Then $P_k$ is an $r_k$-net for all $k$.
%\end{lemma}
%
%\begin{proof}
%    Clearly $P_n$ is an $r_n$-net, so suppose that $k < n.$ Then $P_k$ has coverage radius $r_k$ since $d(p_{k+1}, P_k) = d_H(P_k, P).$ Suppose now that $1 \leq i < j \leq k$. Then $d(p_i,p_j) \geq d(p_j, P_{j-1})$ since $p_i \in P_{j-1}.$ $d(p_j, P_{j-1}) \geq d(p_{k+1}, P_{j-1})$ since $p_j$ is the farthest point in $P$ from $P_{j-1}.$ $d(p_{k+1}, P_{j}) \geq d(p_{k+1}, P_k) = r_k$ because $P_j \subset P_k.$ Hence, $d(p_i, p_j) \geq r_k$. Because $p_i$ and $p_j$ are arbitrary, this implies that the minimum separation of $P_k$ with respect to $P$ is at least $r_k$. Hence, $P_k$ is an $r_k$-net.
%\end{proof}
%
%\begin{definition}
%    Let $P$ be a set of $n$ points. A \textbf{hierarchical tree} on $P$ is a levelled tree $T$ whose vertices are each associated with a point in $P$. The lowest level of the tree contains $n$ leaf vertices, each of which is associated with a unique point in $P$. Every vertex in the tree is uniquely identifiable by its point in $P$ and its level in $T$. The vertex associated with a point $p$ and level $k$ is denoted by $p^k \in T$. The parent of a vertex $p^k$ is on level $k+1$, and is denoted by $par(p^k)$. The children of a vertex $p^k$ are on level $k-1$ and are denoted by $ch(p^k).$ Every non-leaf vertex must have a nested child associated with the same point. That is, $|ch(p^k)| \geq 1$ implies $p^{k-1} \in ch(p^k).$ $L_k$ denotes the set of points associated with vertices in level $k$ and above.
%    %$P_{p^k}$ denotes the set of points associated with the leaves of the subtree rooted at $p^k.$ 
%\end{definition}
%
%\begin{definition}
%    Let $P$ be a set of $n$ points. A \textbf{cover tree} on $P$ is a hierarchical tree $T$ such that
%
%    \begin{itemize}
%        \item[(i)] \textbf{(Covering condition)} $ch(p^k) \subset B(p, 2^k)$ for all $p^k \in T$, and
%        \item[(ii)] \textbf{(Separating condition)} $\mathcal{S}(L_k) > 2^k$ for all levels $k$.
%    \end{itemize}
%
%    $T$ is called a \textbf{relaxed cover tree} if the separating condition is replaced with:
%
%    \begin{itemize}
%        \item[(ii)] \textbf{(Relaxed separating condition)} $\mathcal{S}(ch(p^{k+1})) > 2^k$ for all $p^{k+1} \in T$.
%    \end{itemize}
%\end{definition}
%
%\begin{lemma}
%    The descendants of a vertex $p^k$ in a cover tree are within a distance of $2^{k+1}$ of $p$.
%\end{lemma}
%
%\begin{proof}
%    The path from the $p^k$ to any descendant $q^{k-l}$ involves a sequence of $l$ vertices $p^k=q_1^k, q_2^{k-1}, \ldots, q_l^{k-l} = q^{k-l}$. By covering condition and triangle inequality, we have
%    $$d(p,q) \leq d(q_1^k,q_2^{k-1}) + \cdots + d(q_{l-1}^{k-l+1}, q_l^{k-l}) \leq 2^k + 2^{k-1} + \cdots \leq 2^{k+1}.$$
%\end{proof}
%
%\section{Literature}
%
%
%\section{Theory}
%
%The motivating application of our research is the construction of a nearest neighbor graph on a finite metric space. A \textbf{metric space} is a pair $(M,d)$ where $M$ is a set of points and $d : M \times M \to [0,\infty)$ is a distance function satisfying $d(x,y) \geq 0$ (\emph{inequality is strict if and only if $x \neq y$}), $d(x,y) = d(y,x)$ and $d(x,y) \leq d(x,z) + d(z,y)$ (\emph{triangle inequality}).
%Our goal is to construct a high-performance distributed-memory data structure that takes a finite metric space $M$ of $n$ points as input, and answers \textbf{metric range queries}: given some $q \in M$ and some radius $r \geq 0$, compute the set of all points in the \textbf{(closed) ball}: $$B(q,r) = \{p \in M : d(p,q) \leq r\}.$$
%Querying every point in $M$ produces a \textbf{nearest neighbor graph} $G_r(M) = (M, E_r(M))$ where $$E_r(M) = \{(p,q) : d(p,q) \leq r\}.$$
%The \textbf{expansion constant} of $M$ is the minimum value $c$ such that $$|B(p,2r)| \leq c\cdot|B(p,r)|$$ for all $p \in M$ and $r > 0.$
%We say that $M$ is a \textbf{growth restricted} metric space if $c$ is constant with respect to $n$. The \textbf{doubling constant} of $M$ is the minimum value $\rho$ such that every ball in $M$ can be covered by $2^\rho$ balls of half the radius. The \textbf{doubling dimension} of $M$ is defined to be $\gamma = \lg{\rho}$.
%
%A \textbf{cover tree} is a data structure that helps answer metric range queries efficiently on a given set of points. Let $(M,d)$ be a finite metric space of $n$ points that we want to build a cover tree for.
%In a cover tree, each vertex has an associated point in $M$ and a level, which counts down from the root to the leaves. Every point in $M$ has a corresponding leaf in the tree. The leaves of the tree are on level $-\infty$, and the root of the tree is on level $+\infty$.
%A point can be associated with multiple internal vertices (non-leaf vertices).
%Each vertex is uniquely determined by its associated point and level.
%The vertex on level $l \in \mathbb{Z} \cup \{-\infty, +\infty\}$ associated with point $p \in M$ is denoted by $p^l.$
%The parent of a vertex $p^l$ is denoted by $par(p^l)$, and its children are denoted by $ch(p^l).$ Child vertices of $p^l$ are on level $l-1$. Each non-leaf vertex must have a child vertex associated with the same point. This is called the \textbf{nesting invariant}, and we call said child vertex the \emph{nested child} of its parent. Furthermore there are two invariants that must be maintained. The \textbf{covering invariant} stipulates that the children of a vertex on level $l$ are all within a distance of $2^l$ of that vertex. There is also the \textbf{separating invariant}, of which there are two versions. The \emph{global separating invariant} requires all vertices on level $l$ to be pairwise separated by a distance of more than $2^l.$
%The \emph{local separating invariant} requires all sibling vertices on level $l$ (vertices with the same parent on level $l+1$) to be pairwise separated by a distance of more than $2^l.$
%The global separating invariant enables good worst-case bounds, but is difficult to parallelize. We therefore will adopt the global separating invariant to build the replication tree, but the local trees cann only satisfy the local invariant.
%
%Formally, we have the following:
%
%\begin{definition}
%    A \textbf{cover tree} $T$ on a finite set of $n$ metric points $M$ is a levelled tree with $n$ leaves, whose vertices $p^l$ are uniquely identified by their level $l$ and their associated point $p$. The root is on level $\infty$ and the leaves, each of which is associated with one of the points in $M$, are on level $-\infty.$ In addition, the following invariants are maintained (either (iii) or (iv) are true depending on the version but not both):
%    \begin{itemize}
%        \item[(i)] \textbf{(Nesting)} $p^k \in T$ implies $p^{k-1} \in ch(p^k)$,
%        \item[(ii)] \textbf{(Covering)} $ch(p^k) \subseteq B(p, 2^k)$, and
%        \item[(iii)] \textbf{(Local Separating)} $d(q_1,q_2) > 2^{k}$ for all $q^{k}_1 \neq q^{k}_2 \in ch(p^{k+1}).$
%        \item[(iv)] \textbf{(Global Separating)} $d(q_1,q_2) > 2^{k}$ for all $q^k_1 \neq q^k_2$.
%    \end{itemize}
%\end{definition}
%
%Suppose we want to insert a point $p$ into a cover tree $T$ on the set $M$ to form an updated cover tree $T'$ on the set $M \cup \{p\}.$ Let $C^k$ denote the set of vertices on level $k$. Let $Q^k = C^k \cap B(p, 2^{k+1}).$ $Q^k$ is the set of vertices on level $k$ that could be descendants of $p$. This follows because the distance between any vertex on level $k$ and one of its descendants is bounded by $2^{k+1}.$ Let $$R^{k-1} = \bigcup_{q^k \in Q^k}ch(q^k) \subset C^{k-1}$$ be the set of all children of vertices in $Q^k.$
%Let $i$ be any level such that $d(p, R^{i-1}) > 2^i$. Then $d(p, Q^i) > 2^i$ because $Q^i \subset R^{i-1}$ by the nesting property. Note that $d(p,Q^i) = d(p, C^i \cap B(p, 2^{i+1})) > 2^i$ implies $d(p,C^i) > 2^i$, since $d(p, C^i) \leq 2^i$ implies the existence of some point in $C^i$ within a distance of $2^i$, and thus also $2^{i+1},$ of $p$. Therefore $d(p,R^{i-1}) > 2^i$ implies that $d(p, C^i) > 2^i$ and therefore $p$ can be inserted on level $i$ without violating the global separation condition. We therefore find the highest level $i$ for which this is true and attempt to find a parent vertex $q^{i+1} \in Q^{i+1}$ that satisfies the covering condition $d(p,q) \leq 2^{i+1}.$ If no such vertex exists, then we have $d(p,Q^{i+1}) > 2^{i+1}$ which, by the same analysis implies that the separation condition is not violated if we insert $p$ on level $i+1.$ We therefore continue climbing levels until we find a parent. If we don't find a parent at that level, then we know we aren't violating the separation condition above. We keep doing this until we find a parent.
%
%\begin{lemma}
%    All descendant vertices of a vertex $p^k$ represent a point within a distance of $2^{k+1}$ of $p$.
%\end{lemma}
%
%\begin{proof}
%Let the path from $p^k$ on level $k$ to any descendant vertex be $p^k, q^{k-1}_1, \ldots, q^{k-l}_l$. Then
%$$d(p, q_l) \leq d(p^k, q^{k-1}_1) + \cdots + d(q^{k-l+1}_{l-1}, q^{k-l}_l) \leq 2^k(1 + 1/2 + 1/4 + \cdots) = 2^{k+1}.$$
%\end{proof}
%
%\begin{lemma}
%    The number of children of any vertex in a cover tree is at most $c^4.$
%\end{lemma}
%
%\section{Tree}
%
%Let $P_m$ be a greedy permutation that is a prefix of $P$ and that is an $r$-net. Let $V_i = \{p \in P : d(p, p_i) = d(p, P_m)\}$ for $0 \leq i \leq m.$ Each $V_i$ is distributed to a processor, meaning that all the points in $V_i$ are stored locally on a processor.
%For each point $p \in V_i$, we want to compute $B(p,\epsilon).$ However, there may be points $q \in P$ with $d(p,q) \leq \epsilon$ yet $q \notin V_i.$ Hence, if we build a local cover tree just on $V_i$, we don't get $B(p, \epsilon)$, we get $B(p, \epsilon) \cap V_i.$ We therefore need to find all points in other Voronoi cells that could be $\epsilon$-neighbors of points $p \in V_i.$ Let $V_j$ be some Voronoi cell. Query the replication tree for each $p \in V_j$, looking for
%
%\begin{lemma}
%~\cite{karger02}
%If $d(p,q) \leq r$, then $$B(q,r) \subset B(p,2r) \subset B(q,4r).$$
%\end{lemma}
%\begin{proof}
%$x \in B(q,r)$ implies $d(x,q) \leq r$, so that $d(p,x) \leq d(p,q) + d(q,x) \leq 2r.$ Continuing, $x \in B(p, 2r)$ implies $d(q,x) \leq d(p,q) + d(p,x) \leq r + 2r < 4r.$
%\end{proof}
%
%\begin{definition}
%    Let $P$ be a set in a metric space. An $r$-net for $P$ is a subset $S \subset P$ such that $d(p,q) \geq r$ for all $p \neq q \in S$ and $$P \subset \bigcup_{p \in S}B(p,r).$$
%\end{definition}
%
%\subsection{Sunday, March 16}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{|c|l|}
%\hline
%\multicolumn{1}{|l|}{Symbol} & Meaning                      \\ 
%    \hhline{|=|=|}
%$C^k$   & Set of vertices on level $k$ \\
%$l_k+1$ & Number of vertices on level $k$ \\
%$u^k_i$ & The $i$th vertex in $C^k$, where $0 \leq i \leq l_k$ \\
%$f_k : C_k \to C_{k-1}$ & Mapping between vertices and their parents \\
%$S^k_i$ & Set of child vertices of $u^k_i$ \\
%$D^k_i$ & Set of descendant vertices of $u^k_i$ \\
%$n^k_i$ & Number of non-nested children of $u^k_i$ \\
%$N^k_i$ & The sum $n^k_0 + \cdots + n^k_{i}$ \\
%$V^k_i$ & The Voronoi cell of $u^k_i$ induced by the set of vertices in $C^k$ \\
%$r^k_i$ & The maximum distance between $u^k_i$ and a point in $V^k_i$ \\
%$\mathcal{S}(P)$ & The minimum separation of $P$ \\
%$\mathcal{C}(S,P)$ & The coverage radius of $S \subseteq P$ \\
%$\Pi_i(P, p_0)$ & The prefix $\{\pi_0, \ldots, \pi_i\} \subset P$ of a greedy permutation of $P$ such that $p_0 = \pi_0 \in P$ \\
%
%%$(X,d)$                                  & Metric space \\
%%$P$                                      & Point set \\
%%$n = |P|$                                & Total number of points \\
%%$T = T(P)$                               & Cover tree for $P$ \\
%%$B(p,r)$                                 & Metric ball $\{x \in P : d(p,x) \leq r\}$ \\
%%$H(u)$                                   & Hub associated with vertex $u \in T$ \\
%%$\pt(u)$                                 & $\pt(u) = \pi_0(H(u))$ where $u \in T$ \\
%%$\radius(u)$                             & $\radius(u) = r(H(u))$ where $u \in T$ \\
%%$\gamma$                                 & Hub splitting ratio \\
%\end{tabular}
%\vspace{3pt}
%\caption{Symbol Definitions}
%\vspace{-13pt}
%\end{table}
%
%
%\subsection{Friday, March 14}
%
%%Let $Q \subseteq P$ and define $$Q_\epsilon = \bigcup_{q \in Q}B(q,\epsilon).$$
%%It then follows that $$\min\{\epsilon \geq 0 : P \subseteq Q_\epsilon\} = \max_{p \in P}d(p, Q).$$
%%To prove this, observe that for any $r$ such that $P \subseteq Q_r$, we must have that $d(p,Q) \leq r$ for all $p \in P$, because $P \subseteq Q_r$ means that every point in $P$ is in a ball whose center is in $Q$ and whose radius is $r$. Because this is true for all $p \in P$, we have that $P \subseteq Q_r$ implies $\max_{p \in P}d(p,Q) \leq r.$ Suppose $r$ is the minimum value such that $P \subseteq Q_r.$  Then $r' = \max_{p \in P}d(p,Q) \geq r$, for otherwise 
%
%\begin{lemma}
%    $P \subseteq Q_\epsilon$ if and only if $\max_{p \in P}d(p,Q) \leq \epsilon.$
%\end{lemma}
%
%\begin{proof}
%    Suppose $P \subseteq Q_\epsilon$. Then for all $p \in P$, there exists $q \in Q$ such that $d(p,q) \leq \epsilon.$ Hence, $d(p,Q) \leq \epsilon$ for all $p \in P$, which implies $\max_{p\in P}d(p,Q) \leq \epsilon.$ Now suppose $\max_{p \in P}d(p,Q) \leq \epsilon.$ Then $d(p,Q) \leq \epsilon$ for all $p \in P$.
%    This implies that $P \subseteq Q_\epsilon.$
%\end{proof}
%
%\begin{lemma}
%Let $Q \subseteq P$. Then $$\min\{\epsilon \geq 0 : P \subseteq Q_\epsilon\} = \max_{p \in P}d(p, Q).$$
%We call this value the \textbf{coverage radius} of $Q$ with respect to $P$, and it is also written $$d_H(Q,P).$$
%\end{lemma}
%
%\begin{proof}
%    Let $r$ be the minimum value such that $P \subseteq Q_r$ and let $r' = \max_{p \in P}d(p,Q).$ Since $P \subseteq Q_r$, we must have $r' \leq r$. For sake of contradiction, suppose that $r' < r.$ Then $\max_{p \in P}d(p,Q) \leq r'$ implies $P \subseteq Q_{r'}$, which contradicts our selection of $r'$. It follows that $r' \geq r$ and therefore $r = r'$.
%\end{proof}
%
%\begin{definition}
%    $P_k = \{p_1, \ldots, p_k\}$ is a \textbf{greedy permutation} of $P$ (where $1\leq k \leq |P|)$  if $d(p,P_k) \leq d(p_{k+1},P_k)$ for all $p \in P$ and for all $1 \leq k < |P|$.
%\end{definition}
%
%\begin{lemma}
%    Suppose $P$ is ordered by a greedy permutation. Then for all $k$, $P_k$ is an $r$-net where $r = d_H(P_k,P).$
%\end{lemma}
%
%\begin{proof}
%    Note that $d_H(P_k,P) = \max_{p \in P}d(p,P_k) = d(p_{k+1},P_k)$ follows directly. Continuing, let $1 \leq j < i \leq k.$ Then $d(p_i,p_j) \geq d(p_i, P_{i-1}) = d_H(P_{i-1},P)$. Furthermore, $d_H(P_{i-1},P) = \max_{p \in P}d(p,P_{i-1}) \geq \max_{p \in P}d(p, P_i) = d_H(P_i,P).$ By repeatedly applying the last inequality for larger consecutive $i$, we obtain $d_H(P_{i-1}, P) \geq d_H(P_k, P).$ This completes the result.
%\end{proof}
%
%\subsection{Monday, January 20}
%
%Let $(X,d)$ be a finite metric space and $P \subseteq X$ a subset of sites. For each site $p \in P$ we define its corresponding Voronoi cell
%$$V(p) = \{x \in X: d(x,p) = d(x,P)\}.$$
%We also define a neighbor graph $G$ with vertices incident to $P$ and undirected edges $ab \in G$ required if there exists $a' \in V(a)$ and $b' \in V(b)$ such that $d(a', b') \leq d(b', b).$ As the edges are undirected, this is also equivalent to the condition $$d(a', b') \leq \max{\{d(a',a), d(b',b)\}}$$
%for some $a' \in V(a)$ and $b' \in V(b).$
%Essentially, a neighbor graph has an edge from $a$ to $b$ if there exists a point in $V(a)$ closer to some point in $V(b)$ than the latter point is to $b$.
%
%Suppose that we insert a new point $a'$ into the set of sites $P$ to form an updated set of sites $\hat{P}.$ Analogously to before, define
%$$\hat{V}(p) = \{x \in X : d(x,p) = d(x,\hat{P})\}$$
%and $\hat{G}$ is the updated neighbor graph.
%Assuming that the new point $a'$ we are inserting was in the cell $V(a)$, where do we look to find the set of 
%
%%Let $(X,d)$ be a finite metric space and $P = \{p_1, \ldots, p_m\} \subset X$ a subset of $m$ sites of $X$. Let
%%$$V_i = \{x \in X : d(x,p_i) = d(x,P)\}$$
%%for $1 \leq i \leq m$. Let $G = (P, E)$ be a graph such that $(i,j) \in E$ implies that there exists $a \in V_i$ and $b \in V_j$ such that $$d(a,b) < d(b, p_j).$$
%%
%%\emph{In words: $p_j$ is a neighbor of $p_i$ if there is a point in $V_i$ closer to a point $b \in V_j$ than $b$ is to $p_j$. That is, $p_j$ is a neighbor of $p_i$ if adding a new site that is currently in $V_i$ may require stealing points away from $V_j$.}
%%
%%Suppose we want to add a new site $p_{m+1}$ to form the updated subset $\hat{P} = P \cup \{p_{m+1}\}$ and updated Voronoi cells:
%%$\hat{V}_i = \{x \in X : d(x, p_i) = d(x, \hat{P})\}$ for $1 \leq i \leq m+1.$ Furthermore, we create a new graph $\hat{G} = (\hat{P},\hat{E})$ defined analogously for the updated sets. We want a relatively efficient algorithm to do this operation.
%%Adding a new site involves finding the points that should belong to $\hat{V}_{m+1}$ and removing them from their original cells $V_i$ to form $\hat{V}_i$ for $1 \leq i \leq m.$ Let's assume that $p_{m+1}$ was in cell $V_k$ where $1 \leq k \leq m$ is fixed. Consider a point $a \in V_i$ that moves to $\hat{V}_{m+1}.$ This implies that $d(p_{m+1}, a) < d(a, p_i),$ since it means that $a$ is closer to its new nearest site $p_{m+1}$ than to its previous nearest site $p_i.$ Note that this also implies that $(k,i) \in E.$ This means we only have to search the points in the cells $V_i$ for which $(k,i) \in E$ in order to find the points that move to $\hat{V}_{m+1}.$ 
%%\\
%%
%%This tells us how to update the Voronoi cells, but we also need to update $G$ to be $\hat{G}$.
%%We added the new vertex $p_{m+1}$, so that's easy. We will need to compute the neighbors of $p_{m+1}$ in the new graph, as well as potentially deleting edges that no longer satisfy the invariant.
%%$p_j$ will be a neighbor of $p_{m+1}$ if adding a new site in $\hat{V}_{m+1}$ may require stealing points away from $\hat{V}_j.$
%
%\subsection{Thursday, January 16}
%
%Throughout, we assume that $(X,d)$ is a metric space and that $P \subset X$ is a set of $n$ metric points $p_0, \ldots, p_{n-1}$ of interest.
%
%\begin{definition}
%    A \textbf{hierarchical tree} $T$ on the set of points $P$ is a tree whose leaves correspond one-to-one to the points in $P$.
%\end{definition}
%
%
%\section{Cover Tree}
%\subsection{Sunday, January 12}
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P \subseteq X$ a set of points. An $r$-\textbf{net} for $P$ is a subset $S \subseteq P$ such that every point in $P$ is within a distance $r$ of some point in $S$, and such that every pair of distinct points in $S$ is at least $r$ away from each other. In mathematical notation, this is equivalent to
%    \begin{itemize}
%        \item $P \subseteq \bigcup_{x \in S}B(x,r)$; and
%        \item $d(x,y) \geq r$ for all $x \neq y \in S.$
%    \end{itemize}
%\end{definition}
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P = \{p_0, \ldots, p_{n-1}\} \subset X$ a finite set $n$ points from $X$. A \textbf{cover tree} $T = T(P) = (V(T), E(T))$ on the set of points $P$ is a tree such that every tree vertex is associated with a point via the mapping $p : V(T) \to P$, so that, for instance, $p(v) = p_i$ denotes the fact that vertex $v \in V(T)$ is associated with point $p_i \in P.$ Furthermore, there are a set of semantic constraints to be maintained. Each vertex $v$ has a level, such that the parent of $v$ is one level below $v$ and the children of $v$ are one level above. We denote the set of vertices at level $k$ by $C_k$. Note that the root vertex $u_{root} \in V$ is not required to belong to a specific level. We then have the following invariants:
%    \begin{itemize}
%        \item (\textbf{Nesting}) For all $u \in V$ such that $u$ is not childless, there must exist a unique child $v \in V$ such that $p(u) = p(v).$ We call $v$ the nested child vertex of $u$;
%        \item (\textbf{Covering}) Given $u \in C_k$, every child vertex $v$ of $u$ must satisfy $d(u,v) \leq (1/2)^k$.
%        \item (\textbf{Separating}) For every pair of distinct vertices $v_1,v_2 \in C_k$, we must have $d(v_1, v_2) > (1/2)^k.$
%    \end{itemize}
%\end{definition}
%
%For simplicity sake, we make all following arguments under the assumption that $\max_{p \in P}d(p,u_{root}) = 1.$ This has no effect on the correctness of our arguments as we can scale everything appropriately without breaking anything.
%
%We structure our tree further as follows. As already noted, $u_{root} \in V$ denotes the root of $T$ and let $p(u_{root}) = \pi_0 \in P.$ Let $p(S) = \{p(v) : v \in S\}$ where $S \subseteq V$ is a set of vertices. Observe that, because $P \subseteq B(\pi_0, 1),$ we must have $C_0 = \{u_{root}\}.$ We denote the set of children of $u_{root}$ by $u^{1}_0, \ldots u^{1}_{l_1}.$ This means that $C_1 = \{u^{1}_{i}\}_{0 \leq i \leq l_1}.$ By the separating and covering properties, it follows that $p(C_1)$ is a $1/2$-net for $P$. In general, we define $$C_k = \{u^k_{0}, \ldots, u^k_{l_k}\}$$ and observe that $p(C_k)$ is a $(1/2)^k$-net for $P$. Let $S(u)$ denote the set of children of $u$, and let $P(u)$ denote the parent of $u$, which is undefined for $u_{root}.$
%By our current definitions, it follows that
%$$C_{k+1} = \{u^{k+1}_0, \ldots, u^{k+1}_{l_{k+1}}\} = S(u^k_0) \cup \cdots \cup S(u^k_{l_k})$$
%where the union is disjoint.
%In general, it is highly difficult to maintain the full separation condition from a algorithmic complexity point of view. We therefore introduce a relaxed version where the separation condition applies only to sibling vertices with the same parents, but not between all vertices on the same level.
%We therefore introduce the following relaxed version of a net:
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P = \{p_0, \ldots, p_{n-1}\} \subset X$ a finite set of $n$ points from $X$. An $r$-\textbf{cover} for $P$ is a subset $S = \{s_0, \ldots, s_{m-1}\} \subseteq P$ such that $$P \subseteq \bigcup_{i=0}^{m-1}B(s_i, r),$$
%    and such that $d(x,y) > r/2$ for all $x \neq y \in V_i$, where
%    $$V_i = \{p \in P : d(p, s_i) \leq d(p, s_j) \text{ for all $j \neq i$}\}.$$
%\end{definition}
%
%%\begin{definition}
%%    A subset $S \subseteq P$ is called a $(S_1, \ldots,S_m)$-\textbf{cover} for $P$ if $S$ is equal to the disjoint union $S_1 \cup \cdots \cup S_m$, $P \subseteq \cup_{x \in S}B(x,r)$, and such that for every $S_i$ we have $d(x,y) \geq r$ for all $x \neq y \in S_i.$
%%\end{definition}
%%
%%Note that the only difference between this and an $r-net$ is 
%
%\subsection{Monday, January 13}
%
%\begin{align*}
%    C^0 &= \{u^0_0\} \\
%    C^1 &= \{u^1_0, \ldots, u^1_{l_1}\} \\
%    C^2 &= \{u^2_0, \ldots, u^2_{l_1}, \ldots, u^2_{l_2}\} \\
%    &\vdots \\
%    C^k &= \{u^k_0, \ldots, u^k_{l_1}, \ldots, u^k_{l_2}, \ldots, u^k_{l_k}\} \\
%\end{align*}
%$f_k : C^k \to C^{k-1}$ such that $f_k(u^k_i) = u^{k-1}_i$ for $0 \leq i \leq l_{k-1}.$ \\
%$V(u^k_i) = H_i^{l_k} = \{pl\in P : d(p, p_i) \leq d(p,p_j) \text{ for all } 0 \leq j \leq l_k\}$ \\
%$H_i^{l_k} \cap C^k.$
%
%\begin{definition}
%    Let $P = \{p_0, \ldots, p_{n-1}\}$ be a set of $n$ points from a metric space. A $(p_0, \gamma)$-\textbf{prefix} of $P$ is a subset $\Pi = \{\pi_0, \ldots, \pi_{m-1}\}$ of $m$ points from $P$ such that $\pi_0 = p_0$, $d(\pi_{i+1}, \Pi_i) \geq d(p, \Pi_i)$ for all $p \in P$, and $d(p,$
%\end{definition}
%
%\subsection{Tuesday, January 14}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{|c|l|}
%\hline
%\multicolumn{1}{|l|}{Symbol} & Meaning                      \\ 
%    \hhline{|=|=|}
%$C^k$   & Set of vertices on level $k$ \\
%$l_k+1$ & Number of vertices on level $k$ \\
%$u^k_i$ & The $i$th vertex in $C^k$, where $0 \leq i \leq l_k$ \\
%$f_k : C_k \to C_{k-1}$ & Mapping between vertices and their parents \\
%$S^k_i$ & Set of child vertices of $u^k_i$ \\
%$D^k_i$ & Set of descendant vertices of $u^k_i$ \\
%$n^k_i$ & Number of non-nested children of $u^k_i$ \\
%$N^k_i$ & The sum $n^k_0 + \cdots + n^k_{i}$ \\
%$V^k_i$ & The Voronoi cell of $u^k_i$ induced by the set of vertices in $C^k$ \\
%$r^k_i$ & The maximum distance between $u^k_i$ and a point in $V^k_i$ \\
%$\mathcal{S}(P)$ & The minimum separation of $P$ \\
%$\mathcal{C}(S,P)$ & The coverage radius of $S \subseteq P$ \\
%$\Pi_i(P, p_0)$ & The prefix $\{\pi_0, \ldots, \pi_i\} \subset P$ of a greedy permutation of $P$ such that $p_0 = \pi_0 \in P$ \\
%
%%$(X,d)$                                  & Metric space \\
%%$P$                                      & Point set \\
%%$n = |P|$                                & Total number of points \\
%%$T = T(P)$                               & Cover tree for $P$ \\
%%$B(p,r)$                                 & Metric ball $\{x \in P : d(p,x) \leq r\}$ \\
%%$H(u)$                                   & Hub associated with vertex $u \in T$ \\
%%$\pt(u)$                                 & $\pt(u) = \pi_0(H(u))$ where $u \in T$ \\
%%$\radius(u)$                             & $\radius(u) = r(H(u))$ where $u \in T$ \\
%%$\gamma$                                 & Hub splitting ratio \\
%\end{tabular}
%\vspace{3pt}
%\caption{Symbol Definitions}
%\vspace{-13pt}
%\end{table}
%
%Structurally, a cover tree is a tree whose vertices correspond to a finite set of points in a given metric space. The root vertex is assumed to be on level $0$, and the children of vertices on level $k$ are on level $k+1.$ All vertices except for those on the level with the highest index are assumed to have a unique \emph{nested child}, which is a vertex that corresponds to the same point as its parent. Hence, all vertices except for those on the highest level have at least one child. Let $C^k$ denote the set of vertices on level $k$. Let $l_k + 1$ denote the number of vertices in $C^k$. We assume an ordering of the vertices on each level such that $u^k_i$ represents the $i$th vertex on level $k$, so that $$C^k = \{u^k_0, u^k_1, \ldots, u^k_{l_k}\}.$$
%Vertices represent the same point if and only if they share a subscript, e.g. $u^k_i$ and $u^{k+1}_i$ represent the same point, on levels $k$ and $k+1$, respectively. By this setup, it follows that $u^{k+1}_i$ is the nested child of $u^k_i$, as it represents the same point, is on the level just above, and because nested children are unique.
%Let $n^k_i$ denote the number of non-nested children of $u^k_i,$ and let $N^k_i = n^k_0 + \cdots + n^k_i.$ For each $k$, let $f_k : C^k \to C^{k-1}$ map each level $k$ vertex to its parent vertex, and let $S^{k-1}_i = f^{-1}_k(u^{k-1}_i) \subset C^k$ denote the set of children vertices of $u^{k-1}_i.$ We adopt an ordering of the child vertices such that
%$$S^k_i = f^{-1}_{k+1}(u^k_i) = \{u^{k+1}_i, u^{k+1}_{l_k + N^k_{i-1} + 1}, \ldots, u^{k+1}_{l_k + N_i^k}\}$$
%for all $0 \leq i \leq l_k.$
%In this ordering, we always put the nested children at the beginning of each level, and then fill in the non-nested children for each vertex by its corresponding order in the parent level.
%Using these definitions, it follows that $l_{k+1} = l_k + N_{l_k}^k$ and $l_0 = 0.$ We assume that the tree has $M+1$ levels and that every point in our finite set has at least one corresponding vertex in the tree. It follows that $C^M$ contains one vertex for each point, and therefore the number of points in the finite set is $n = l_M + 1.$
%
%\begin{definition}
%    Let $P \subseteq X$ be a finite set of points from some metric space. The \textbf{minimum separation} of $P$, denoted $\mathcal{S}(P)$, is the smallest distance between pairwise distinct points in $P$. That is,
%    $$\mathcal{S}(P) = \min_{p \neq q \in P}d(p, q).$$
%\end{definition}
%
%\begin{definition}
%    Let $P \subseteq X$ be finite. The \textbf{coverage radius} of a subset $S \subseteq P$ is the minimum $r$ such that $$P \subseteq \bigcup_{x \in S}B(x,r).$$
%    We let $\mathcal{C}(S,P)$ denote the coverage radius of $S$ with respect to $P$.
%\end{definition}
%
%\begin{definition}
%    A subset $S \subseteq P$ is an $(\alpha, \beta)$-\textbf{net} if $\mathcal{S}(S) \geq \alpha$ and $\mathcal{C}(S,P) \leq \beta.$ $S$ is called an $\alpha$-\textbf{net} if it is an $(\alpha, \alpha)$-net.
%\end{definition}
%
%With this setup, we may now introduce the semantic definition of the classic cover tree.
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P \subseteq X$ a finite subset of $n$ points. A \textbf{cover tree} $T = T(P)$ on the set of points $P$ is a tree with the above structural definition and the following invariants:
%
%    \begin{itemize}
%        \item[(i)] \textbf{Covering}. $S^k_i \subseteq B(u^k_i, r/2^k)$, where $r$ is a dataset specific constant large enough so that all points can be reached from the root; and
%        \item[(ii)] \textbf{Separating}. $d(u^k_i, u^k_j) > r/2^k$ for all $0 \leq i < j \leq l_k.$
%    \end{itemize}
%\end{definition}
%
%Note that the separating condition is equivalent to stating that $\mathcal{S}(C^k) > r/2^k.$
%
%\begin{lemma}
%    $C^k$ is an $(r/2^k, r/2^{k-1})$-net for $P$.
%\end{lemma}
%
%\begin{proof}
%    The minimum separation for $C^k$ is greater than $r/2^k$ by definition. Furthermore, we can write $C^k$ as a union of the child sets from $C^{k-1}$, namely
%    $$C^k = S^{k-1}_0 \cup S^{k-1}_1 \cup \cdots \cup S^{k-1}_{l_{k-1}}.$$
%    By the covering condition, it follows that
%    $$C^k \subseteq \bigcup_{i=0}^{l_{k-1}}B(u^{k-1}_i, r/2^{k-1}),$$
%    implying that $\mathcal{C}(C^k,P) \leq r/2^{k-1}.$ Therefore, $C^k$ is an $(r/2^k, r/2^{k-1})$-net.
%\end{proof}
%
%We will now introduce a few more notational conveniences. We assume an ordering on the set of points $P$ that is consistent with the ordering of tree vertices, so that $u^0_i, \ldots, u^k_i$ all correspond to the same point $p_i \in P$, where $0 \leq i \leq l_k.$ Since we assume that $T$ has $M$ levels, it follows that $P = \{p_0, \ldots, p_{l_M}\}.$
%Let $V^k_i$ denote the Voronoi cell induced by the set of vertices on level $k$. That is, let
%$$V_i^k = \{p \in P : d(p, p_i) \leq d(p, p_j) \text{ for all } 0 \leq i < j \leq l_k\}.$$
%Let $r^k_i = \max_{p \in V^k_i}d(p, p_i)$ be the farthest distance between $u^k_i$ and a point in its Voronoi cell. Let $D^k_i$ denote the set of all descendants of $u^k_i.$ By repeated application of the covering property, we have the following lemma:
%
%\begin{lemma}
%$$D^k_i \subseteq B(p_i, r/2^{k-1}).$$
%\end{lemma}
%
%\begin{proof}
%    Perhaps fill in later. It's not too hard to show.
%\end{proof}
%
%We now introduce two alternative versions of the cover tree that are easier to deal with.
%
%\begin{definition}
%    We call a cover tree $T$ \textbf{condensed} if $$D^k_i \subseteq B(p_i, r/2^k).$$
%\end{definition}
%
%For a condensed cover tree, we assume that $r = \max_{p \in P}d(p,p_0)$.
%
%\begin{definition}
%    We call a cover tree $T$ \textbf{relaxed} if the separation condition is adjusted to be that $$\mathcal{S}(S^{k-1}_i) > r/2^k$$ for all $0 \leq i \leq l_{k-1}.$
%\end{definition}
%
%Note that the difference between a relaxed cover tree and a normal cover tree is that in the normal cover tree, we require all vertices on level $k$ to be separated by $r/2^k,$ whereas in the relaxed tree we only require vertices with the same parent to satisfy the condition with respect to each other. We do not prohibit points on the same level with different parents from being within a distance of $r/2^k.$
%
%Let us now consider the recursive cover tree construction algorithm I have been utilizing so far. I believe it will turn out that we are not actually satisfying all the cover tree properties, and this may lead to excessive load imbalance in the distributed-memory implementation. We start with the notion of a greedy permutation.
%
%\begin{definition}
%    Let $P \subseteq X$ be a set of $n$ points from a metric space. Consider an ordering $(\pi_0, \ldots, \pi_{n-1})$ of the points of $P$, where $\Pi_i = \{\pi_0, \ldots, \pi_i\}$ denotes the prefix consisting of the first $i+1$ points of the ordering. The ordering is called a \textbf{greedy permutation} if $d(\pi_i,\Pi_{i-1}) \geq d(p, \Pi_{i-1})$ for all $p \in P$ and all $1 \leq i \leq n-1.$ We call the ordering a $c$-\textbf{approximate greedy permutation} if the condition is replaced with $c\cdot d(\pi_i, \Pi_{i-1}) \geq d(p, \Pi_{i-1}),$ where $c \geq 1$ is a constant.
%\end{definition}
%
%\begin{lemma}
%    Let $(\pi_0, \ldots, \pi_{n-1})$ be a greedy permutation ordering of $P$, and define $r_k = d(\pi_{k+1},\Pi_k)$ for $0 \leq k \leq n-2$ and $r_{n-1} = 0.$ Then $\Pi_k$ is an $r_k$-net for $P$ for all $k$.
%\end{lemma}
%
%\begin{proof}
%    For any $\pi_i \neq \pi_j \in \Pi_k$ we can assume without loss of generality that $0 \leq i < j \leq k.$ Therefore $d(\pi_i, \pi_j) \geq d(\pi_j, \Pi_{j-1}) = r_{j-1}$. Furthermore, note that $r_i$ is a decreasing sequence since $$r_i = d(\pi_{i+1}, \Pi_i) \geq d(\pi_{i+1},\Pi_{i-1}) \geq d(\pi_{i}, \Pi_{i-1}) = r_{i-1}.$$
%    Hence, $r_{j-1} \geq r_k$ and therefore $d(\pi_i, \pi_j) \geq r_k.$
%    In addition, for any $p \in P$, there exists $\pi_i \in \Pi_k$ such that $d(p, \pi_i) = d(p, \Pi_k) \leq d(\pi_{k+1}, \Pi_k) = r_k.$
%\end{proof}
%
%A similar argument shows that for a $c$-approximate greedy permutation, $\Pi_k$ is a $(r_k/c, r_k)$-net. 



%\section{Nearest Neighbors}
%
%\subsection{Friday, January 10}
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P \subseteq X$ a set of points. An $r$-\textbf{net} for $P$ is a subset $S \subseteq P$ such that every point in $P$ is within a distance $r$ of some point in $S$, and such that every pair of distinct points in $S$ is at least $r$ away from each other. In mathematical notation, this is equivalent to
%    \begin{itemize}
%        \item $P \subseteq \bigcup_{x \in S}B(x,r)$; and
%        \item $d(x,y) \geq r$ for all $x \neq y \in S.$
%    \end{itemize}
%\end{definition}
%
%\begin{definition}
%    Let $(X,d)$ be a metric space and $P \subseteq X$ a set of $n$ points. A \textbf{greedy permutation} on $P$ is an ordering $(p_1, \ldots, p_n)$ of the points of $P$ such that $d(p_{i+1}, P_i) \geq d(p, P_i)$ for all $p \in P$, where $P_i = (p_1, \ldots, p_i)$.
%\end{definition}
%
%\begin{lemma}
%    Let $(p_1, \ldots, p_n)$ be a greedy permutation of $P \subseteq X$ and define $r_k = d(p_{k+1}, P_k).$ Then $P_k$ is an $r_k$-net for $P$ for all $1 \leq k \leq n-1.$ 
%\end{lemma}
%
%\begin{proof}
%\end{proof}
%
%\section{Persistent Homology}
%
%\subsection{Tuesday, January 7}
%
%\newcommand{\comp}{\mathcal{S}}
%
%An \textbf{(abstract) simplicial complex} is a pair $K = (V, \comp)$ where $V$ is finite set of \textbf{vertices} and $\comp$ is a collection of nonempty finite subsets of $V$, called \textbf{simplices} (singular \textbf{simplex}), that satisfy the following two properties:
%
%\begin{itemize}
%    \item $v \in V \Rightarrow \{v\} \in \comp,$ and
%    \item $\sigma \in \comp$ and $\tau \subseteq \sigma \Rightarrow \tau \in \comp.$ 
%    %\item $\tau \subseteq \sigma \in \comp \Rightarrow \tau \in \comp.$
%\end{itemize}
%
%The \textbf{dimension} of a simplex $\sigma \in \comp$ is defined to be $\dim{\sigma} = |\sigma| - 1$. A $p$-dimensional simplex is called a \textbf{$p$-simplex}. If $\tau \subseteq \sigma \in \comp$ then we call $\tau$ a \textbf{face} of $\sigma$ and $\sigma$ a \textbf{coface} of $\tau$; another way to define a simplicial complex is therefore a set of vertices such that every vertex is associated with a corresponding $0$-simplex in $\comp$ and such that the faces of any simplex in $\comp$ must also be in $\comp$. An \textbf{ordering} of a $p$-simplex $\sigma$ is a sequence of its $p+1$ vertices, $\sigma = [v_0, v_1, \ldots, v_p].$ We write $[\sigma]$ when we want to stress that $\sigma$ has an ordering.
%An \textbf{orientation} is an equivalence class of orderings such that two orderings (which are permutations) are equivalent if and only if they both have an even number of transpositions.
%The sign of a permutation is $+1$ if the permutation has an even number of transpositions and it is $-1$ otherwise.
%We say $[\sigma]$ is positively oriented (positive) if its ordering is even and negative if it is odd.
%Every permutation of $2$ or more elements is either even or odd, hence every $p$-simplex with $p \geq 1$ is either positive or negative, and every $0$-simplex is positive. Note that if $[\sigma] = [v_0,v_1, \ldots, v_p]$ and $[\tau] = [v_{\pi(0)}, v_{\pi(1)}, \ldots, v_{\pi(p)}]$, where $\pi$ is a permutation, then $[\sigma] = [\tau]$ if $\pi$ is even and $[\sigma] = -[\tau]$ if $\pi$ is odd. The \textbf{dimension} of a complex $K$ is the maximum dimension of any of its simplices. A \textbf{subcomplex} is a simplicial complex $K'= (V, \comp')$ where $\comp' \subseteq \comp.$ The \textbf{$p$-skeleton} of a complex $K$ is the largest subcomplex of dimension $p$.
%
%\begin{definition}
%    A \textbf{metric space} is a pair $(X,d)$ where $X$ is a set of points and $d : X \times X \to \mathbb{R}^{\geq0}$ is a \textbf{distance} function such that
%    \begin{itemize}
%        \item $d(x,y) \geq 0$ for all $x,y \in X$,
%        \item $d(x,y) = 0$ if and only if $x = y$,
%        \item $d(x,y) = d(y,x)$ for all $x,y \in X$, and
%        \item $d(x,y) \leq d(x,z) + d(z,y)$ for all $x,y,z \in X.$
%    \end{itemize}
%\end{definition}
%
%Our algorithms all assume a finite input set $P \subset X$ of $n$ points.
%Throughout our analysis we make use of the metric ball, defined for point $p$ and radius $r$ to be the set of points $$B(p,r) \eqdef \{p \in P : d(p,x) \leq r\}.$$
%Notice that we use $P$ as the universe within $B(p,r)$ resides, not $X$.
%
%\begin{definition} A \textbf{hub} is a triple $(H,\pi_0,r)$ where
%\begin{itemize}
%    \item $H \subset P$ is a subset of points,
%    \item $\pi_0 \in H$ is the \textbf{hub representative} of $H$, and
%    \item $r \eqdef \max_{p \in H}d(p,\pi_0)$ is the \textbf{hub radius} of $H$.
%\end{itemize}
%Associated with a hub is its \textbf{hub ball} $$B(H) \eqdef B(\pi_0, r) = \{p \in P : d(p,\pi_0) \leq r\}.$$
%\end{definition}
%Note that the hub ball for $H$ may (and often does) contain points outside of $H$. When it is not explicitly clear which representative or radius we are referring to, we write $\pi_0(H)$ and $r(H)$ to clarify.
%
%Hubs are utilized to facilitate cover tree construction. For each hub $H$, there is an associated tree vertex $u \in T$ where $\pt(u) = \pi_0(H).$
%The complete set of points associated with the descendants of $u$ are none other than the set of points in $H$.
%
%The key primitive we require is a splitting function which selects child hub representatives $\pi_0, \pi_1, \ldots, \pi_{m} \in H$ that induce child hubs $(H_0, \pi_0, r_0), \ldots, (H_m, \pi_m, r_m)$
%such that
%$$H_i = \{p \in H : d(p,\pi_i) \leq d(p,\pi_j) \text{ for all } i \neq j\},$$
%and the following invariants are maintained:
%\begin{itemize}
%    \item[(1)] \textbf{Covering}. $H \subset \bigcup_{i=0}^{m}B(\pi_i, r/2),$
%    \item[(2)] \textbf{Separating}. $d(\pi_i, \pi_j) > r/2$ for all $i \neq j.$
%\end{itemize}
%We then insert vertices $v_0, v_1, \ldots, v_m$ into $T$ as children of $u$, with $\pt(v_i) = \pi_i$.
%Note that we always select $\pi_0$ as a child hub representative to maintain the nesting invariant.
%In practice, it is not required to maintain $r/2$ as the splitting radius. For example, a value of $r/1.3$ was found by~\cite{izbicki15} to have superior performance in their experiments.
%To be flexible, we define a \emph{splitting ratio} $1/2 \leq \gamma < 1$ to be a floating parameter that can be adjusted to better fit certain datasets.
%Our splitting function is outlined in Algorithm~\ref{alg:hub_split}.

%\begin{table}[h]
%\centering
%\begin{tabular}{|c|l|}
%\hline
%\multicolumn{1}{|l|}{Symbol} & Meaning                      \\ 
%    \hhline{|=|=|}
%
%$(X,d)$                                  & Metric space \\
%$P$                                      & Point set \\
%$n = |P|$                                & Total number of points \\
%$T = T(P)$                               & Cover tree for $P$ \\
%$B(p,r)$                                 & Metric ball $\{x \in P : d(p,x) \leq r\}$ \\
%$H(u)$                                   & Hub associated with vertex $u \in T$ \\
%$\pt(u)$                                 & $\pt(u) \eqdef \pi_0(H(u))$ where $u \in T$ \\
%$\radius(u)$                             & $\radius(u) \eqdef r(H(u))$ where $u \in T$ \\
%$\gamma$                                 & Hub splitting ratio \\
%\end{tabular}
%\vspace{3pt}
%\caption{Symbol Definitions}
%\vspace{-13pt}
%\end{table}

%\begin{algorithm}
%\caption{Hub splitting algorithm}
%\label{alg:hub_split}
%\begin{algorithmic}[1]
%\Require
%\begin{itemize}
%    \item Parent hub $(H, \pi_0, r)$
%    \item Distance array $D$ initialized with $D[p] \gets d(p, \pi_0)$ for all $p \in H$,
%    \item Candidate representative $\pi_1 = \argmax_{p \in H}D[p]$ \Comment{Note that $r = D[\pi_1]$}
%    \item Splitting ratio $1/2 \leq \gamma < 1.$
%\end{itemize}
%\Ensure
%\begin{itemize}
%    \item Child hubs $(H_0, \pi_0, r_0), \ldots, (H_m, \pi_m, r_m)$,
%    \item Distance arrays $D_0, \ldots, D_m$ with $D_i[p] = d(p, \pi_i)$ for all $p \in H_i$
%\end{itemize}
%with
%\begin{itemize}
%    \item[(1)] \textbf{Covering}. $H \subset \bigcup_{i=0}^m B(\pi_i, \gamma \cdot r)$,
%    \item[(2)] \textbf{Separating}. $d(\pi_i, \pi_j) > \gamma \cdot r$ for all $i \neq j$.
%\end{itemize}
%\Function{SplitHub}{$H$, $D$, $\pi_0$, $\pi_1$, $\gamma$}
%    \State $L[p] \gets \pi_0$ for all $p \in H$
%    \BeginBox
%    \State $m \gets 0$
%    \Repeat
%        \State $m \gets m + 1$
%        \State $D^{*}[p] \gets d(p, \pi_m)$ for all $p \in H$
%        \For{$p \in H$}
%            \If {$D^{*}[p] < D[p]$}
%                \State $D[p] \gets D^{*}[p]$
%                \State $L[p] \gets \pi_m$
%            \EndIf
%        \EndFor
%        \State $\pi_{m+1} \gets \argmax_{p \in H}D[p]$
%    \Until{$D[\pi_{m+1}] \leq \gamma \cdot r$} \Comment{$\pi_{m+1}$ violates separating condition}
%    \EndBox
%    \BeginBox
%    \For{$i \gets 0..m$}
%        \State $H_i \gets \{p \in H : L[p] = \pi_i\}$
%        \State $D_i[p] \gets D[p]$ for all $p \in H_i$
%        \State $\pi_1(H_i) \gets \argmax_{p \in H_i}D_i[p]$ \Comment{Note that $\pi_1(H_i)$ is not $\pi_1$}
%        \State $r_i \gets D_i[\pi_1(H_i)]$
%        \State $(H_i, \pi_i, r_i)$ is a child hub with distance array $D_i$ and candidate representative $\pi_1(H_i)$
%    \EndFor
%    \EndBox
%\EndFunction
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%\caption{Level construction algorithm}
%\label{alg:build_level}
%\begin{algorithmic}[1]
%\Require
%\begin{itemize}
%    \item Cover tree $T$ with $l$ levels completed,
%    \item $\mathrm{Hubs} = \{H^{(i)}, \pi_{0}^{(i)}, \pi_{1}^{(i)}, r^{(i)}, u_i\}_{1 \leq i \leq m}$ where $u_i$ is parent vertex of hub $(H^{(i)}, \pi_{0}^{(i)}, r^{(i)}),$
%    \item Splitting ratio $1/2 \leq \gamma < 1,$
%    \item Minimum hub size $\zeta \geq 1$
%\end{itemize}
%\Ensure Cover tree $T$ with $l+1$ levels completed
%\Function{BuildLevel}{$T$, $\mathrm{Hubs}$, $\gamma$, $\zeta$}
%    \For {$i \gets 1..m$}
%        \State $\{H^{(i)}_j\}_{1 \leq j \leq m_i}$  \\
%        $\gets$ \Call{SplitHub}{$H^{(i)}$, $D^{(i)}, \pi_{0}^{(i)}, \pi_{1}^{(i)}, \gamma$}
%        \State $\mathrm{Hubs} \gets \mathrm{Hubs} \setminus \{H^{(i)}\}$
%        \For{$j \gets 1..m_i$}
%            \State Insert vertex $v = B(\pi_0(H_{j}^{(i)}), r_{j}^{(i)})$ with parent $u_i$
%            \If{$|H_{j}^{(i)}| > \zeta$}
%                \State $\mathrm{Hubs} \gets \mathrm{Hubs} \cup \{H_{j}^{(i)}\}$
%            \Else
%                \If{$|H_{j}^{(i)}| > 1$}
%                    \For {$p \in H_{j}^{(i)}$}
%                        \State Insert leaf vertex $B(p,0)$ with parent $v$
%                    \EndFor
%                \EndIf
%            \EndIf
%        \EndFor
%    \EndFor
%\EndFunction
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%\caption{Distributed memory cover tree construction}
%\label{alg:dist_cover_Tree}
%\begin{algorithmic}[1]
%\State 
%\end{algorithmic}
%\end{algorithm}
%
%
%\begin{algorithm}
%\caption{Fixed-radius nearest neighbor query}
%\label{alg:point_query}
%\begin{algorithmic}[1]
%\Require
%\begin{itemize}
%    \item Cover tree $T = T(P)$,
%    \item Query point $q \in X$,
%    \item Neighborhood query radius $\epsilon \geq 0$.
%\end{itemize}
%\Ensure The set of $\epsilon$-neighbors of $q$: $N = B(q, \epsilon) \subset P.$
%\Function{BallQuery}{$T, q, \epsilon$}
%    \State $N \gets \varnothing$
%    \State $S \gets \{T_{\mathrm{root}}\}$ \Comment{$T_\mathrm{root}$ is the root vertex of $T$}
%    \While{$S \neq \varnothing$}
%        \State $u \gets \textsc{PopBack}(S)$
%        \If{$\textsc{IsLeaf}(u)$ and $d(q, \pt(u)) \leq \epsilon$}
%            \State $N \gets N \cup \{\pt(u)\}$
%        \Comment{If we are searching for ghost hubs, the \textsc{IsLeaf} condition returns true if $u$ is an active hub representative, and we replace the distance comparison condition with $d(q,\pt(u)) \leq \radius(u) + \epsilon$}
%        \Else
%            \For{$v \in \textsc{Children}(u)$} 
%                \If{$d(q, \pt(v)) \leq \radius(v) + \epsilon$}
%                    \State $\textsc{PushBack}(S, v)$
%                \EndIf
%            \EndFor
%        \EndIf
%    \EndWhile
%    \Return $N$
%\EndFunction
%\end{algorithmic}
%\end{algorithm}
%
%Check out paper~\cite{karger02}

==> table/table-datasets.tex <==
\begin{table}[h!]
\centering
\caption{Point clouds}
\label{tab:point_clouds}
\begin{tabular}{lcccc|rrr}
\toprule
Dataset & Metric & Dimension & Points & Size & $\epsilon$-radius & Edges & Avg. neighbors\\
\midrule
\multirow{8}*{\textbf{faces}} & \multirow{8}*{Euclidean} & \multirow{8}*{$20$} & \multirow{8}*{$10304$} & \multirow{8}*{$845$KB} & $95.66$ & $3.81$M & $370.31$ \\
& & & & & $106.29$ & $5.61$M & $543.99$\\
& & & & & $118.10$ & $8.09$M & $785.34$\\
& & & & & $131.22$ & $11.44$M & $1111.03$\\
& & & & & $145.80$ & $15.81$M & $1534.26$\\
& & & & & $162.00$ & $21.32$M & $2068.62$\\
& & & & & $180.00$ & $27.95$M & $2712.62$\\
& & & & & $200.00$ & $35.29$M & $3424.50$\\
\midrule
\multirow{8}*{\textbf{artificial40}} & \multirow{8}*{Euclidean} & \multirow{8}*{$40$} & \multirow{8}*{$10000$} & \multirow{8}*{$1.6$MB} & $6.70$ & $1.12$M & $112.47$ \\
& & & & & $6.87$ & $1.82$M  & $182.14$\\
& & & & & $7.05$ & $2.88$M  & $287.88$\\
& & & & & $7.23$ & $4.43$M  & $443.03$\\
& & & & & $7.41$ & $6.64$M  & $663.57$\\
& & & & & $7.61$ & $9.67$M  & $966.68$\\
& & & & & $7.80$ & $13.69$M & $1368.51$\\
& & & & & $8.00$ & $18.80$M & $1880.15$\\
\midrule
\multirow{8}*{\textbf{corel}} & \multirow{8}*{Euclidean} & \multirow{8}*{$32$} & \multirow{8}*{$68040$} & \multirow{8}*{$8.6$MB} & $0.033$ & $199$K & $2.93$ \\
& & & & & $0.044$ & $290$K & $4.26$ \\
& & & & & $0.059$ & $454$K & $6.68$ \\
& & & & & $0.079$ & $821$K & $12.07$ \\
& & & & & $0.105$ & $1.98$M & $29.03$ \\
& & & & & $0.141$ & $6.64$M & $97.56$ \\
& & & & & $0.188$ & $27.15$M & $399.06$ \\
& & & & & $0.250$ & $113.42$M & $1667.02$ \\
\midrule
\multirow{8}*{\textbf{covtype}} & \multirow{8}*{Euclidean} & \multirow{8}*{$55$} & \multirow{8}*{$581012$} & \multirow{8}*{$124$MB} & $119.57$ & $27.20$M & $46.82$ \\
& & & & & $132.86$ & $37.68$M & $64.86$ \\
& & & & & $147.62$ & $53.25$M & $91.65$ \\
& & & & & $164.03$ & $76.44$M & $131.57$ \\
& & & & & $182.25$ & $111.49$M & $191.88$ \\
& & & & & $202.50$ & $164.91$M & $283.83$ \\
& & & & & $225.00$ & $246.91$M & $424.97$ \\
& & & & & $250.00$ & $372.92$M & $641.85$ \\
\midrule
\textbf{twitter} & Euclidean & $78$ & $583250$ & $176$MB\\
\midrule

\bottomrule
\end{tabular}
\end{table}
